Evaluating Voice Skills by Design Guidelines Using an Automatic Voice Crawler

Currently, adaptive voice applications supported by voice assistants (VA) are very popular (i.e., Alexa skills and Google Home Actions). Under this circumstance, how to design and evaluate these voice interactions well is very important. In our study, we developed a voice crawler to collect responses from 100 most popular Alexa skills under 10 different categories and evaluated these responses to find out how they comply with 8 selected design guidelines published by Amazon. Our findings show that basic commands support are the most followed ones while those related to personalised interaction are relatively less. There also exists variation in design guidelines compliance across different skill categories. Based on our findings and real skill examples, we offer suggestions for new guidelines to complement the existing ones and propose agendas for future HCI research to improve voice applications' user experiences.

==> 4-studies.tex <==
\section{Studies}
%\subsection{User Experience Testing}
Based on the Amazon's voice design guide\cite{GuideA}, we chose 13 key design features from 4 aspects that we would like to test and came up with corresponding testing commands used for crawler loops. By following these commands, we collected the corresponding responses and did a series of analysis to show current situations of the selected design guidelines' compliance. The details are shown as follows.
\subsection{Basic commands support:} Basic commands of Alexa skills include "open", "help" and "stop". A user can start using a certain skill by saying "Alexa, open" plus the name of the skill and when a user wants to know the skill instructions or stop using the skill, they can say "Alexa, help" or "Alexa, stop". For basic commands support testing, we designed crawler loops by setting the commands as basic commands. Within one round of the crawler loop, the crawler will first give "open", "help", "stop" commands and then listen to the responses in turn, after that convert them into text. Based on the responses collected, we can know how many skills support basic commands and conduct our analysis.
\subsection{Remember what was said:} According to the design guide, users will greatly appreciate it if skills could remember what was said by users before and provided more personalized services. In order to test whether the skill could remember what was said and provided corresponding responses, we conducted our crawler loop testing after the skill was interrupted in the middle of use. Then we would analyze the responses collected to see whether the skill remember last interaction and change it's responses
accordingly. 

\subsection{Problem handling support:} Problem handling is one of the most important parts in user interface design. When evaluating Alexa skills design, we choose several problem handling scenarios, one is how the Alexa skill will respond when it receives no answers from user and the other is when Alexa skill cannot understand the commands from user. When we tested the first scenario, we chose to use basic commands first and then stopped giving command to wait for how the skill would respond. For the second scenario, we came up with some meaningless commands like "blah blah" and garbled to collect the responses.

\subsection{Natural language responses support}
\begin{itemize}
  
   
   
    \item \textbf{Variety support} Using variety can inject a natural and less robotic feel into a conversation and make repeat interactions sound less rote or memorized. In this case, we focused on testing language variations under repeat interactions where users give "open", "help" and "stop" command. We designed to use crawler loops three times with basic commands under different situations. The first time of the crawler loop would be run when these Alexa skills are enabled in the first time; the second round of crawler loop would be played under the situation where these skills have already been explored and the the third round would be run after the skill was interrupted in the middle of use. 
    \item \textbf{Conversational markers support:} When users converse, they tend to use some conversational markers to make their expression more understandable. As a conversational agent, Alexa skills also need to include conversational markers to talk more naturally. In our test, we focused on these four kinds of conversational markers: timeline markers like "First", "halfway there", "then", "last"; acknowledgement and feedback, like "Okay", "Got it", "thank you"; pointers like "this", "that", "it's"; transitions like "Now", "so", "all right". In order to evaluate conversational markers support situation, we put all our collected data together to check the appearance of conversational markers.
\end{itemize}


